BraTS-Path Challenge: Assessing Heterogeneous Histopathologic Brain Tumor Sub-regions

Glioblastoma is the most common primary adult brain tumor, with a grim prognosis - median survival of 12-18 months following treatment, and 4 months otherwise. Glioblastoma is widely infiltrative in the cerebral hemispheres and well-defined by heterogeneous molecular and micro-environmental histopathologic profiles, which pose a major obstacle in treatment. Correctly diagnosing these tumors and assessing their heterogeneity is crucial for choosing the precise treatment and potentially enhancing patient survival rates. In the gold-standard histopathology-based approach to tumor diagnosis, detecting various morpho-pathological features of distinct histology throughout digitized tissue sections is crucial. Such "features" include the presence of cellular tumor, geographic necrosis, pseudopalisading necrosis, areas abundant in microvascular proliferation, infiltration into the cortex, wide extension in subcortical white matter, leptomeningeal infiltration, regions dense with macrophages, and the presence of perivascular or scattered lymphocytes. With these features in mind and building upon the main aim of the BraTS Cluster of Challenges https://www.synapse.org/brats2024, the goal of the BraTS-Path challenge is to provide a systematically prepared comprehensive dataset and a benchmarking environment to develop and fairly compare deep-learning models capable of identifying tumor sub-regions of distinct histologic profile. These models aim to further our understanding of the disease and assist in the diagnosis and grading of conditions in a consistent manner.

==> Notes.tex <==
# Important notes/TODO for manuscript goes here 

Synapse is a collaborative research platform that helps teams share, organize, and discuss their scientific research.  Synapse supports the capacity to create and manage community data challenges, using containerized models for secure evaluation of participant submitted methods.


%\and Dominic LaBella\inst{1,\dag,\ddag,\S,\P,*,\orcid{0000-0003-1713-9538}}
%\and Maruf Adewole\inst{2,\dag}
%\and Michelle Alonso-Basanta\inst{3,\dag,\ddag,\S}
%\and Talissa Altes\inst{4,\dag}
%\and Syed Muhammad Anwar\inst{5,6,\dag}
%\and Timothy Bergquist\inst{10,\dag}
%\and Radhika Bhalerao\inst{11,\dag}
%\and Sully Chen\inst{12,\dag}
%\and Byrone Cole\inst{10,\dag}
%\and Gian-Marco Conte\inst{13,\dag}
%\and Farouk Dako\inst{14,\dag}
%\and Maria Diaz\inst{10,\dag}
%\and Ivan Ezhov\inst{15,16,\dag}
%\and Devon Godfrey\inst{1,\dag}
%\and Fathi Hilal\inst{4,\ddag}
%\and Ariana Familiar\inst{17,\dag}
%\and Keyvan Farahani\inst{18,\dag}
%\and Juan Eugenio Iglesias\inst{19,\dag}
%\and Zhifan Jiang\inst{5,6,\dag}
%\and Elaine Johanson\inst{20,\dag}
%\and Anahita Fathi Kazerooni\inst{7,17,\dag}
%\and Collin Kent\inst{1,\dag}
%\and John Kirkpatrick\inst{1,\ddag}
%\and Florian Kofler\inst{15,16,21,22,\dag}
%\and Koen Van Leemput\inst{23,\dag}
%\and Hongwei Bran Li\inst{19,24,25,\dag}
%\and Xinyang Liu\inst{5,6,\dag}
%\and Aria Mahtabfar\inst{26,\dag, \ddag,\S}
%\and Shan McBurney-Lin\inst{11,\ddag}
%\and Ryan McLean\inst{27,\dag,\ddag,\S}
%\and Zeke Meier\inst{28,\dag}
%\and Ahmed W Moawad\inst{29,\dag}
%\and John Mongan\inst{11,\ddag}
%\and Pierre Nedelec\inst{11,\ddag,\S}
%\and Maxence Pajot\inst{11,\ddag,\S}
%\and Marie Piraud\inst{21,\dag}
%\and Arif Rashid\inst{3,\ddag}
%\and Zachary Reitman\inst{1,\dag,\ddag}
%\and Russell Takeshi Shinohara\inst{7,30,\dag}
%\and Yury Velichko\inst{31,\dag}
%\and Chunhao Wang\inst{1,\dag,\ddag}
%\and Pranav Warman\inst{12,\dag}
%\and Walter Wiggins\inst{32,\dag,\ddag}
%\and Mariam Aboian\inst{27,\dag,\ddag,\S,\P}
%\and Jake Albrecht\inst{10,\dag,\P}
%\and Udunna Anazodo\inst{33,\dag,\P}
%\and Adam Flanders\inst{26,\dag,\P}
%\and Anastasia Janas\inst{27,\dag,\S,\P}
%\and Goldey Khanna\inst{26,\dag,\ddag,\S,\P}
%\and Marius George Linguraru\inst{5,6,\dag,\P}
%\and Bjoern Menze\inst{24,25,\dag,\P}
%\and Ayman Nada\inst{4,\dag,\ddag,\S,\P}
%\and Andreas M Rauschecker\inst{11,\dag,\ddag,\S,\P}
%\and Jeffrey D. Rudie\inst{11,34,\dag,\S,\P}
%\and Nourel Hoda Tahon\inst{4,\dag,\ddag,\S,\P}
%\and Javier Villanueva-Meyer\inst{11,\dag,\ddag,\S,\P}
%\and Benedikt Wiestler\inst{24,\dag,\P}
%\and Evan Calabrese\inst{32,\dag,\ddag,\S,\P,**}
%}
 Department of Radiation Oncology, Duke University Medical Center, Durham, NC, USA
\and Medical Artificial Intelligence (MAI) Lab, Crestview Radiology, Lagos, Nigeria
\and Department of Radiation Oncology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA
\and Missouri University, Columbia, MO, USA 
\and Children's National Hospital, Washington DC, USA
\and George Washington University, Washington DC, USA
\and Center for AI and Data Science for Integrated Diagnostics (AI2D) and Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA, USA
\and Department of Radiology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA
\and Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA
\and University of California San Francisco, CA, USA
\and Duke University Medical Center, School of Medicine, USA
\and Center for Global Health, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA
\and Department of Informatics, Technical University Munich, Germany
\and TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany
\and Children’s Hospital of Philadelphia, University of Pennsylvania, Philadelphia, PA, USA
\and Cancer Imaging Program, National Cancer Institute, National Institutes of Health, Bethesda, MD 20814, USA
\and Athinoula A Martinos Center for Biomedical Imaging, Massachusetts General Hospital, Boston, MA, USA
\and PrecisionFDA, U.S. Food and Drug Administration, Silver Spring, MD, USA
\and Helmholtz AI, Helmholtz Munich, Germany
\and Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany
\and Department of Applied Mathematics and Computer Science, Technical University of Denmark, Denmark
\and Department of Neuroradiology, Technical University of Munich, Munich, Germany
\and University of Zurich, Switzerland
\and Department of Neurosurgery, Thomas Jefferson University, Philadelphia, PA, USA 
\and Yale University, New Haven, CT, USA
\and Booz Allen Hamilton, McLean, VA, USA
\and Mercy Catholic Medical Center, Darby, PA, USA
\and Center for Clinical Epidemiology and Biostatistics, University of Pennsylvania, Philadelphia, USA
\and Department of Radiology, Northwestern University, Evanston, IL, USA
\and Department of Radiology, Duke University Medical Center, Durham, NC, USA 
\and Montreal Neurological Institute (MNI), McGill University, Montreal, QC, Canada
\and University of San Diego, CA, USA

